A Multiscale Environment for Learning by Diffusion

Clustering algorithms partition a dataset into groups of similar points. The clustering problem is very general, and different partitions of the same dataset could be considered correct and useful. To fully understand such data, it must be considered at a variety of scales, ranging from coarse to fine. We introduce the Multiscale Environment for Learning by Diffusion (MELD) data model, which is a family of clusterings parameterized by nonlinear diffusion on the dataset. We show that the MELD data model precisely captures latent multiscale structure in data and facilitates its analysis. To efficiently learn the multiscale structure observed in many real datasets, we introduce the Multiscale Learning by Unsupervised Nonlinear Diffusion (M-LUND) clustering algorithm, which is derived from a diffusion process at a range of temporal scales. We provide theoretical guarantees for the algorithm's performance and establish its computational efficiency. Finally, we show that the M-LUND clustering algorithm detects the latent structure in a range of synthetic and real datasets.

==> ACHA Manuscript - arXiv-2/cluster_comparisons.tex <==


\subsection{Comparison of Clusterings in $\MESMR$}

By the definition of $\mathcal{I}_\epsilon^{(\ell)}$ and by Corollary \ref{cor:diff_dist_bound}, if  $\delta^{(\ell)}t\leq\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t\leq\frac{\epsilon}{2}$, then the clustering  $\{X_k^{(\ell)}\}_{k=1}^{K_\ell}$ is $\epsilon$-separable by diffusion distances at time $t$. Lemma \ref{lemma: OutInterval} implies that the reason that $\{X_k^{(\ell)}\}_{k=1}^{K_\ell}$ is not $\epsilon$-separable by diffusion distances at times $t\notin \mathcal{I}_\epsilon^{(\ell)}$ may be because exactly one of these conditions fails. So, a MESMR clustering that is not $\epsilon$-separable by diffusion distances at time $t$ will either be well-separated within the original graph but not very coherent, or very coherent but not very well-separated within the original graph. One can interpret the interval $\mathcal{I}_\epsilon^{(\ell)}$ as the time steps during which both of these statements are true. 

\begin{lemma} \label{lemma: OutInterval}
If $t$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$, then $\delta^{(\ell)}t<\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t>\frac{\epsilon}{2}$. If $t$ occurs after $\mathcal{I}_\epsilon^{(\ell)}$, then  $\delta^{(\ell)}t>\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t<\frac{\epsilon}{2}$. 
\end{lemma}
\begin{proof}
If $t$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$, then $t< \frac{\ln(2\kappa^{(\ell)}/\epsilon)}{\ln(1/|\lambda^{(\ell)}_{K_{\ell}+1}|)}$, which reduces to $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t>\frac{\epsilon}{2}$. Also, $t<\frac{\epsilon}{2\delta^{(\ell)}}$, which reduces to $\delta^{(\ell)}t<\frac{\epsilon}{2}$. On the other hand, if $t$ occurs after $\mathcal{I}_\epsilon^{(\ell)}$, then $ \frac{\ln(2\kappa^{(\ell)}/\epsilon)}{\ln(1/|\lambda_{K_\ell+1}^{(\ell)})}<t$, which reduces to  $\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t<\frac{\epsilon}{2}$. Also, $\frac{\epsilon}{2\delta^{(\ell')}}<t$, which reduces to $\frac{\epsilon}{2}<\delta^{(\ell')}t$. \end{proof}

By Theorem \ref{thm:Meyer}, for any $t\geq0$, $\|P^t-[S^{(\ell)}]^\infty\|_\infty<\delta^{(\ell)}t +\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t$ for each $\ell\in\{1,\dots, M\}$. If this bound is small, that would imply that $P^t$ is approximated well by the steady-state multiscale stochastic complement of $P$ corresponding to the $\ell$\ths clustering in $\MESMR$. In this sense, the quantity $\delta^{(\ell)}t +\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t$ can be thought of as a measure of ``goodness of fit'' of the $\ell$\ths clustering in $\MESMR$ at time $t$.  In the following theorem, we show that when $t\in \mathcal{I}_\epsilon^{(\ell)}$, this bound is minimal for the geometric constants associated with the $\ell$\ths clustering. In this sense, the $\ell$\ths clustering in $\MESMR$ is the one that best reflects the latent structure of the data during the interval  $\mathcal{I}_\epsilon^{(\ell)}$.

\begin{theorem}\label{thm: constant argmin}
    Assume that $t\in \mathcal{I}_\epsilon^{(\ell)}$ for a fixed $\epsilon>0$ and $\kappa^{(\ell)} = \kappa^{(\ell')}$. Then $\ell = \text{\emph{argmin}}_{1\leq \ell'\leq M} \big( \delta^{(\ell')}t +\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\big)$. 
\end{theorem}
\begin{proof}
We will prove the statement by contradiction and assume that there is an $\ell'\neq \ell$ such that for some $t\in \mathcal{I}_\epsilon^{(\ell)}$, $\delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\geq \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t$. Because all intervals do not overlap, $\mathcal{I}_\epsilon^{(\ell')}$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$ or after. We will prove that both cases lead to a contradiction. 
\begin{enumerate}
    \item Assume that $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$. By assumption, $ \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\leq\epsilon$, where we have used that $t\in \mathcal{I}_\epsilon^{(\ell)}$ to obtain the last inequality.  As $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$,  Lemma \ref{lemma: OutInterval} implies $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t<\frac{\epsilon}{2}$.  Subtracting this inequality from $\delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \epsilon$, we obtain that $\delta^{(\ell')}t\leq \frac{\epsilon}{2}$ for this choice of $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq \ell$. However, Lemma \ref{lemma: OutInterval} implies that $\delta^{(\ell')}t > \frac{\epsilon}{2}$ for any $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq\ell$. This gives us our contradiction. 

    \item Assume that $\mathcal{I}_\epsilon^{(\ell)}$ occurs before $\mathcal{I}_\epsilon^{(\ell')}$. By assumption, $ \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\leq\epsilon$, where we have used that $t\in \mathcal{I}_\epsilon^{(\ell)}$ to obtain the last inequality.  As $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$,  Lemma \ref{lemma: OutInterval} implies $\delta^{(\ell)}t<\frac{\epsilon}{2}$.  Subtracting this inequality from $\delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \epsilon$, we obtain that $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \frac{\epsilon}{2}$ for this choice of $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq \ell$. However, Lemma \ref{lemma: OutInterval} implies that $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t > \frac{\epsilon}{2}$ for any $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq\ell$. This gives us our contradiction. 
\end{enumerate}
\end{proof}

By Corollary \ref{cor:diff_dist_bound}, for any $t\geq 0$ and $\ell\in \{1,\dots, M\}$, $\frac{D_t^{\text{in}}(\ell)}{D_t^{\text{btw}}(\ell)}\geq\frac{\gamma^{(\ell)}(t)\big(\delta^{(\ell)}t + \kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\big)}{\sqrt{n\pi_{\min}}\min_{w\in X}\|s_\infty^{(\ell)}(w,:)\|_2-\gamma^{(\ell)}(t)\big(\delta^{(\ell)}t + \kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\big)}$. If this bound is small, the clusters in the $\ell$\ths MESMR clustering of $X$ are well-separated by diffusion distances at time $t$. However, for any fixed $t$, this bound will be uninformative (or even trivial) for some clustering scales $\ell$ and imply good separation of clusters in others. Thus, it is of importance to understand how diffusion distances for a fixed time interact with different clusterings in $\MESMR$. Assume that for any $\ell'\neq \ell$ and $t\in \mathcal{I}_\epsilon^{(\ell)}$, that $\gamma^{(\ell)}(t)=\gamma^{(\ell')}(t)$,  $\kappa^{(\ell)}=\kappa^{(\ell')}$, and $\min_{w\in X}\|s_\infty^{(\ell)}(w,:)\|_2=\min_{w\in X}\|s_\infty^{(\ell')}(w,:)\|_2$. Then Theorem \ref{thm: constant argmin} implies that the upper bound on $D_t^{\text{in}}(\ell)/D_t^{\text{btw}}(\ell)$ is minimal for the $\ell$\ths clustering in the MESMR data model. In other words, diffusion distances separate the clusters in the $\ell$\ths clustering better than any other clustering in the MESMR data model when $t\in \mathcal{I}_\epsilon^{(\ell)}$. 



==> cluster_comparisons.tex <==


\subsection{Comparison of Clusterings in $\MESMR$}

By the definition of $\mathcal{I}_\epsilon^{(\ell)}$ and by Corollary \ref{cor:diff_dist_bound}, if  $\delta^{(\ell)}t\leq\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t\leq\frac{\epsilon}{2}$, then the clustering  $\{X_k^{(\ell)}\}_{k=1}^{K_\ell}$ is $\epsilon$-separable by diffusion distances at time $t$. Lemma \ref{lemma: OutInterval} implies that the reason that $\{X_k^{(\ell)}\}_{k=1}^{K_\ell}$ is not $\epsilon$-separable by diffusion distances at times $t\notin \mathcal{I}_\epsilon^{(\ell)}$ may be because exactly one of these conditions fails. So, a MESMR clustering that is not $\epsilon$-separable by diffusion distances at time $t$ will either be well-separated within the original graph but not very coherent, or very coherent but not very well-separated within the original graph. One can interpret the interval $\mathcal{I}_\epsilon^{(\ell)}$ as the time steps during which both of these statements are true. 

\begin{lemma} \label{lemma: OutInterval}
If $t$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$, then $\delta^{(\ell)}t<\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t>\frac{\epsilon}{2}$. If $t$ occurs after $\mathcal{I}_\epsilon^{(\ell)}$, then  $\delta^{(\ell)}t>\frac{\epsilon}{2}$ and $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t<\frac{\epsilon}{2}$. 
\end{lemma}
\begin{proof}
If $t$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$, then $t< \frac{\ln(2\kappa^{(\ell)}/\epsilon)}{\ln(1/|\lambda^{(\ell)}_{K_{\ell}+1}|)}$, which reduces to $\kappa^{(\ell)}|\lambda_{K_{\ell}+1}^{(\ell)}|^t>\frac{\epsilon}{2}$. Also, $t<\frac{\epsilon}{2\delta^{(\ell)}}$, which reduces to $\delta^{(\ell)}t<\frac{\epsilon}{2}$. On the other hand, if $t$ occurs after $\mathcal{I}_\epsilon^{(\ell)}$, then $ \frac{\ln(2\kappa^{(\ell)}/\epsilon)}{\ln(1/|\lambda_{K_\ell+1}^{(\ell)})}<t$, which reduces to  $\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t<\frac{\epsilon}{2}$. Also, $\frac{\epsilon}{2\delta^{(\ell')}}<t$, which reduces to $\frac{\epsilon}{2}<\delta^{(\ell')}t$. \end{proof}

By Theorem \ref{thm:Meyer}, for any $t\geq0$, $\|P^t-[S^{(\ell)}]^\infty\|_\infty<\delta^{(\ell)}t +\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t$ for each $\ell\in\{1,\dots, M\}$. If this bound is small, that would imply that $P^t$ is approximated well by the steady-state multiscale stochastic complement of $P$ corresponding to the $\ell$\ths clustering in $\MESMR$. In this sense, the quantity $\delta^{(\ell)}t +\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t$ can be thought of as a measure of ``goodness of fit'' of the $\ell$\ths clustering in $\MESMR$ at time $t$.  In the following theorem, we show that when $t\in \mathcal{I}_\epsilon^{(\ell)}$, this bound is minimal for the geometric constants associated with the $\ell$\ths clustering. In this sense, the $\ell$\ths clustering in $\MESMR$ is the one that best reflects the latent structure of the data during the interval  $\mathcal{I}_\epsilon^{(\ell)}$.

\begin{theorem}\label{thm: constant argmin}
    Assume that $t\in \mathcal{I}_\epsilon^{(\ell)}$ for a fixed $\epsilon>0$ and $\kappa^{(\ell)} = \kappa^{(\ell')}$. Then $\ell = \text{\emph{argmin}}_{1\leq \ell'\leq M} \big( \delta^{(\ell')}t +\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\big)$. 
\end{theorem}
\begin{proof}
We will prove the statement by contradiction and assume that there is an $\ell'\neq \ell$ such that for some $t\in \mathcal{I}_\epsilon^{(\ell)}$, $\delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\geq \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t$. Because all intervals do not overlap, $\mathcal{I}_\epsilon^{(\ell')}$ occurs before $\mathcal{I}_\epsilon^{(\ell)}$ or after. We will prove that both cases lead to a contradiction. 
\begin{enumerate}
    \item Assume that $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$. By assumption, $ \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\leq\epsilon$, where we have used that $t\in \mathcal{I}_\epsilon^{(\ell)}$ to obtain the last inequality.  As $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$,  Lemma \ref{lemma: OutInterval} implies $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t<\frac{\epsilon}{2}$.  Subtracting this inequality from $\delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \epsilon$, we obtain that $\delta^{(\ell')}t\leq \frac{\epsilon}{2}$ for this choice of $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq \ell$. However, Lemma \ref{lemma: OutInterval} implies that $\delta^{(\ell')}t > \frac{\epsilon}{2}$ for any $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq\ell$. This gives us our contradiction. 

    \item Assume that $\mathcal{I}_\epsilon^{(\ell)}$ occurs before $\mathcal{I}_\epsilon^{(\ell')}$. By assumption, $ \delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \delta^{(\ell)}t+\kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\leq\epsilon$, where we have used that $t\in \mathcal{I}_\epsilon^{(\ell)}$ to obtain the last inequality.  As $\mathcal{I}_\epsilon^{(\ell)}$ occurs after $\mathcal{I}_\epsilon^{(\ell')}$,  Lemma \ref{lemma: OutInterval} implies $\delta^{(\ell)}t<\frac{\epsilon}{2}$.  Subtracting this inequality from $\delta^{(\ell')}t + \kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \epsilon$, we obtain that $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t\leq \frac{\epsilon}{2}$ for this choice of $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq \ell$. However, Lemma \ref{lemma: OutInterval} implies that $\kappa^{(\ell')}|\lambda_{K_{\ell'}+1}^{(\ell')}|^t > \frac{\epsilon}{2}$ for any $t\in \mathcal{I}_\epsilon^{(\ell)}$ and $\ell'\neq\ell$. This gives us our contradiction. 
\end{enumerate}
\end{proof}

By Corollary \ref{cor:diff_dist_bound}, for any $t\geq 0$ and $\ell\in \{1,\dots, M\}$, $\frac{D_t^{\text{in}}(\ell)}{D_t^{\text{btw}}(\ell)}\geq\frac{\gamma^{(\ell)}(t)\big(\delta^{(\ell)}t + \kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\big)}{\sqrt{n\pi_{\min}}\min_{w\in X}\|s_\infty^{(\ell)}(w,:)\|_2-\gamma^{(\ell)}(t)\big(\delta^{(\ell)}t + \kappa^{(\ell)}|\lambda_{K_\ell+1}^{(\ell)}|^t\big)}$. If this bound is small, the clusters in the $\ell$\ths MESMR clustering of $X$ are well-separated by diffusion distances at time $t$. However, for any fixed $t$, this bound will be uninformative (or even trivial) for some clustering scales $\ell$ and imply good separation of clusters in others. Thus, it is of importance to understand how diffusion distances for a fixed time interact with different clusterings in $\MESMR$. Assume that for any $\ell'\neq \ell$ and $t\in \mathcal{I}_\epsilon^{(\ell)}$, that $\gamma^{(\ell)}(t)=\gamma^{(\ell')}(t)$,  $\kappa^{(\ell)}=\kappa^{(\ell')}$, and $\min_{w\in X}\|s_\infty^{(\ell)}(w,:)\|_2=\min_{w\in X}\|s_\infty^{(\ell')}(w,:)\|_2$. Then Theorem \ref{thm: constant argmin} implies that the upper bound on $D_t^{\text{in}}(\ell)/D_t^{\text{btw}}(\ell)$ is minimal for the $\ell$\ths clustering in the MESMR data model. In other words, diffusion distances separate the clusters in the $\ell$\ths clustering better than any other clustering in the MESMR data model when $t\in \mathcal{I}_\epsilon^{(\ell)}$. 


